On critical points of random polynomials and spectrum of certain products of random matrices

In the first part we study critical points of random polynomials. We choose two deterministic sequences of complex numbers,whose empirical measures converge to the same probability measure in complex plane. We make a sequence of polynomials whose zeros are chosen from either of sequences at random. We show that the limiting empirical measure of zeros and critical points agree for these polynomials. As a consequence we show that when we randomly perturb the zeros of a deterministic sequence of polynomials, the limiting empirical measures of zeros and critical points agree. This result can be interpreted as an extension of earlier results where randomness is reduced. Pemantle and Rivin initiated the study of critical points of random polynomials. Kabluchko proved the result considering the zeros to be i.i.d. random variables. In the second part we deal with the spectrum of products of Ginibre matrices. Exact eigenvalue density is known for a very few matrix ensembles. For the known ones they often lead to determinantal point process. Let $X_1,X_2,...,X_k$ be i.i.d matrices of size $n \times n$ whose entries are independent complex Gaussian random variables. We derive the eigenvalue density for matrices of the form $Y_1.Y_2....Y_n$, where each $Y_i = X_i$ or $X_i^{-1}$. We show that the eigenvalues form a determinantal point process. The case where $k=2$, $Y_1=X_1,Y_2=X_2^{-1}$ was derived earlier by Krishnapur. The case where $Y_i =X_i$ for all $i=1,2,...,n$, was derived by Akemann and Burda. These two known cases can be obtained as special cases of our result.

==> poissonginibre3.tex <==
\chapter{Poisson process from spectrum of Ginibre matrices}
\label{ch:PoissonGinibre3}
%Todo: Link the convergence of point processes to the convergence of joint correlation functions.
\section{Introduction}
Let $X_n$ be a complex Ginibre matrix of size $n \times n$, whose entries $X(i,j)$ are i.i.d  $CN(0,\frac{1}{n})$. Let $\lambda_{1,n},\lambda_{2,n},\dots,\lambda_{n,n}$ be the eigenvalues of $X_n$. It is long known that the point process constituted by the eigenvalues of $X_n$ is a determinantal point process with kernel given by $\textbf{$\mathbb{K}$}(z,w)=\sum\limits_{j=0}^{n-1}\frac{(nz\overline{w})^j}{j!}$ w.r.t the reference measure $\frac{1}{\pi}ne^{-n|z|^2}dm(z)$. Let $\mu_{1,n},\mu_{2,n},\dots,\mu_{n,n}$ be the eigenvalues of $X_n^n$ which are related as $\lambda_{k,n}^n=\mu_{k,n}$. In this chapter we will investigate whether the point processes obtained by $\mu_{k,n}$s will converge to some point process as $n \rightarrow \infty$. For this it is enough to check if the $k^{th}$ joint intensity  $\rho_{k,n}'(z_1,z_2,\dots,z_k)$ of $\mu_{\ell,n}$s converge to the corresponding joint intensity of the limiting point process. We will show that the limiting point process is Poisson on $\textbf{$\mathbb{C}$}\backslash \{0\}$ with intensity $f(.)$. As the $k^{th}$ joint intensity of Poisson point process at points $z_1,z_2,\dots,z_k$ is $f(z_1)f(z_2)\dots f(z_k)$, it is enough to show that $\rho_{k,n}'(z_1,z_2,\dots,z_n)$ converge to the same. 

We will show the computational proof of the above fact by demonstrating the proof for $k=1,2$ and later prove for the general $k$.

\section{Preliminaries and results}
\begin{theorem}\label{poissonginibre}
	
\end{theorem}
\section{Proof of Theorem\ref{poissonginibre}}
Let $\omega_n=e^{\frac{2\pi i}{n}}$ is an $n^{th}$root of unity. 
\subsubsection{Case:k=1}
For this case there isn't anything to verify but merely obtain the intensity of the Poisson point process.

\begin{align}
\rho_{1,n}'(z) & = \lim\limits_{\epsilon \rightarrow 0}\dfrac{\Pr\left(\sum\limits_{i=1}^{n}\text{$\mathbbm{1}$}\left(\mu_{i,n}\in B(z,\epsilon)\right)=1 \right)}{\pi\epsilon^2}\\
& =  \lim\limits_{\epsilon \rightarrow 0}\dfrac{\Pr\left(\sum\limits_{i=1}^{n}\sum\limits_{j=1}^{n}\text{$\mathbbm{1}$}\left(\lambda_{i,n}\in B\left(z^{\frac{1}{n}}\omega_n^j,\dfrac{\epsilon}{n|z|^{1-\frac{1}{n} }}+O(\epsilon^2)\right)\right)=1\right)}{\pi\epsilon^2}\\
& = \lim\limits_{\epsilon \rightarrow 0}\dfrac{\Pr\left(\sum\limits_{i=1}^{n}\text{$\mathbbm{1}$}\left(\lambda_{i,n}\in \bigcup\limits_{j=1}^{n}B\left(z^{\frac{1}{n}}\omega_n^j,\dfrac{\epsilon}{n|z|^{1-\frac{1}{n}}}+O(\epsilon^2)\right)\right)=1\right)}{\pi\epsilon^2}\\
& =  \lim\limits_{\epsilon \rightarrow 0}\dfrac{\int\limits_{A_n}\rho_{1,n}(w)dm(w)+O(\epsilon^4)}{\pi\epsilon^2} 
\end{align}
Where $A_n=\bigcup\limits_{j=1}^{n}B\left(z^{\frac{1}{n}}\omega_n^j,\dfrac{\epsilon}{n|z|^{1-\frac{1}{n}}}+O(\epsilon^2)\right)$.
Hence
\begin{align}
\rho_{1,n}(z) & = \dfrac{\sum\limits_{i=1}^{n}\rho_{1,n}(z^\frac{1}{n}\omega_n^j)}{n^2|z|^{2(1-\frac{1}{n})}}= \dfrac{K_n(z^\frac{1}{n},z^\frac{1}{n})}{n|z|^{2-\frac{2}{n}}}\\
& = \sum\limits_{i=0}^{n-1}\dfrac{n^i|z|^\frac{2i}{n}}{i!}\dfrac{e^{-n|z|^\frac{2}{n}}}{\pi|z|^{2-\frac{2}{n}}}\\
& = \dfrac{1}{\pi|z|^{2-\frac{2}{n}}}\sum\limits_{i=0}^{n-1}\dfrac{n^i|z|^\frac{2i}{n}}{i!}e^{-n|z|^\frac{2}{n}}\\
& = \frac{1}{\pi |z|^{2-\frac{2}{n}}}\Pr\left(\sum_{i=1}^{n}P_i^{(|z|^\frac{2}{n})}<n\right)\\
& \text{(where $P_1^{(t)},P_2^{(t)},\dots,P_n^{(t)}$ are i.i.d Poisson(t) random variables)}
\end{align}

Therefore the 1-point intensity of the limiting point process will be $$\rho_1'(z)=\lim\limits_{n\rightarrow\infty}\rho_{1,n}'(z)=\lim\limits_{n\rightarrow\infty}\frac{1}{\pi|z|^2}|z|^\frac{2}{n}\Pr\left(\sum\limits_{i=1}^{n}P_i^{(|z|^\frac{2}{n})}<n\right)=\frac{1}{2\pi|z|^2}$$


\subsubsection{Case:k=2}
\begin{align}
\rho_{2,n}'(z_1,z_2) & = \lim\limits_{\epsilon\rightarrow 0}\dfrac{\Pr\left(\sum\limits_{i=1}^{n}\text{$\mathbbm{1}$}\left(\mu_{i,n}\in B(z_1,\epsilon)\right)=1 \& \sum\limits_{i=1}^{n}\text{$\mathbbm{1}$}\left(\mu_{i,n}\in B(z_2,\epsilon)\right)=1 \right)}{(\pi\epsilon^2)^2}\\
\end{align}
Using the relation $\mu_{i,n}=\lambda_{i,n}^n$ and changing variables  we  obtain that the events $\{\mu_{i,n}\in B(z_1,\epsilon)\}$ and  $\{\lambda_{i,n}\in \bigcup\limits_{j=1}^{n}B(z_1^\frac{1}{n}\omega_n^j,\epsilon_n')\}$ as well as $\{\mu_{i,n}\in B(z_2,\epsilon)\}$ and  $\{\lambda_{i,n}\in \bigcup\limits_{j=1}^{n}B(z_2^\frac{1}{n}\omega_n^j,\epsilon_n'')\}$ are identical for some $\epsilon_n'=\frac{\epsilon}{n|z_1|^{1-\frac{1}{n}}}+O(\epsilon^2)$ and $\epsilon_n''=\frac{\epsilon}{n|z_2|^{1-\frac{1}{n}}}+O(\epsilon^2)$. Hence we have

\begin{align}
\rho_{2,n}'(z_1,z_2)& = \lim\limits_{\epsilon\rightarrow 0} \dfrac{\Pr\left(\sum\limits_{i=1}^{n}\text{$\mathbbm{1}$}\left(\lambda_{i,n}\in \bigcup\limits_{j=1}^{n}B(z_1^\frac{1}{n}\omega_n^j,\epsilon_n')\right)=1 \& \sum\limits_{i=1}^{n}\text{$\mathbbm{1}$}\left(\lambda_{i,n}\in\bigcup\limits_{j=1}^{n} B(z_2^\frac{1}{n}\omega_n^j,\epsilon_n'')\right)=1 \right)}{(\pi\epsilon^2)^2}\\
& = \lim\limits_{\epsilon \rightarrow 0} \dfrac{\int\limits_{A_n\times B_n}\rho_{2,n}(\alpha,\beta)dm(\alpha)dm(\beta)}{(\pi\epsilon^2)^2}
\end{align}
where $A_n=\bigcup\limits_{j=1}^{n}B(z_1^\frac{1}{n}\omega_n^j,\epsilon_n'),B_n=\bigcup\limits_{j=1}^{n}B(z_2^\frac{1}{n}\omega_n^j,\epsilon_n'')$ and $\rho_{2,n}(.,.)$ is the $2^{nd}$ joint intensity of the eigenvalue process of $X_n$. Therefore,

\begin{align}
\rho_{2,n}'(z_1,z_2) &= \dfrac{\sum\limits_{i,j=1}^{n}\left(\rho_{2,n}(z_1^{\frac{1}{n}}\omega_n^i,z_2^\frac{1}{n}\omega_n^j)\right)}{n^4|z_1z_2|^{2-\frac{2}{n}}}\\
&= \frac{1}{n^4|z_1z_2|^{2-\frac{2}{n}}}\sum\limits_{i,j=1}^{n}\left(K(z_1^{\frac{1}{n}}\omega_n^j,z_1^{\frac{1}{n}}\omega_n^i)K(z_2^{\frac{1}{n}}\omega_n^j,z_2^{\frac{1}{n}}\omega_n^j)-K(z_1^{\frac{1}{n}}\omega_n^i,z_2^{\frac{1}{n}}\omega_n^j)K(z_2^{\frac{1}{n}}\omega_n^j,z_1^{\frac{1}{n}}\omega_n^i)\right)\\
&= \frac{1}{n^4|z_1z_2|^{2-\frac{2}{n}}}\left(n^2K(z_1^\frac{1}{n},z_1^\frac{1}{n})K(z_2^\frac{1}{n},z_2^\frac{1}{n})-\sum\limits_{i,j=1}^{n}|K(z_1^\frac{1}{n}\omega_n^i,z_2^\frac{1}{n}\omega_n^j)|^2\right) \label{last2}
\end{align}

We will now show that $\lim\limits_{n\rightarrow\infty}\dfrac{\sum\limits_{i,j=1}^{n}|K(z_1^\frac{1}{n}\omega_n^i,z_2^\frac{1}{n}\omega_n^j)|^2}{n^4|z_1z_2|^{2-\frac{2}{n}}}=0$.

\begin{align}
\sum\limits_{i,j=1}^{n}|K(z_1^\frac{1}{n}\omega_n^i,z_2^\frac{1}{n}\omega_n^j)|^2 & = n^2e^{-n(|z_1|^\frac{2}{n}+|z_2|^\frac{2}{n})}\sum\limits_{i,j=1}^{n}\left(\sum\limits_{\ell=0}^{n-1}(z_1^\frac{1}{n}\omega_n^i\overline{z_2}^\frac{1}{n}\overline{\omega_n}^{j})^\ell\frac{n^\ell}{\ell!}\right)\left(\sum\limits_{\ell=0}^{n-1}(\overline{z_1}^\frac{1}{n}\overline{\omega_n}^{i}z_2^\frac{1}{n}\omega_n^{j})^\ell\frac{n^\ell}{\ell!}\right)\\
& = n^2e^{-n(|z_1|^\frac{2}{n}+|z_2|^\frac{2}{n})}\sum\limits_{i,j=1}^{n}\left(\sum\limits_{\ell,k=1}^{n-1}\frac{\left(z_1^\frac{\ell}{n}\omega_n^{i\ell}\overline{z_2}^\frac{\ell}{n}\overline{\omega_n}^{j\ell}\overline{z_1}^\frac{k}{n}\overline{\omega_n}^{ki}z_2^\frac{k}{n}\omega_n^{kj}\right)n^{k+\ell}}{k!\ell!}\right)\\
& =n^2e^{-n(|z_1|^\frac{2}{n}+|z_2|^\frac{2}{n})}\sum\limits_{i,j=1}^{n}\left(\sum\limits_{\ell,k=1}^{n-1}\frac{n^{k+\ell}}{k!\ell!}\left(\omega_n^{(i-j)(\ell-k)}\right)\left(z_1^\frac{\ell}{n}\overline{z_1}^\frac{k}{n}z_2^\frac{k}{n}\overline{z_2}^\frac{\ell}{n}\right)\right)
\end{align}
Let $z_1=r_1e^{i\theta_1}$, $z_2=r_2e^{i\theta_2}$ and $\alpha=e^{i(\theta_1-\theta_2)}$.
\begin{align}
\sum\limits_{i,j=1}^{n}|K(z_1^\frac{1}{n}\omega_n^i,z_2^\frac{1}{n}\omega_n^j)|^2
& = n^2e^{-n(|z_1|^\frac{2}{n}+|z_2|^\frac{2}{n})}\sum\limits_{i,j=1}^{n}\left(\sum\limits_{\ell,k=0}^{n-1}\frac{n^{k+\ell}}{k!\ell!}\left(\omega_n^{(i-j)(\ell-k)}\right)\alpha^{\ell-k}(r_1r_2)^\frac{\ell+k}{n}\right)\\
& = n^2e^{-n(|z_1|^\frac{2}{n}+|z_2|^\frac{2}{n})}\sum\limits_{\ell\neq k=0}^{n-1}\left(\sum\limits_{i,j=1}^{n}\frac{n^{k+\ell}}{k!\ell!}\left(\omega_n^{(i-j)(\ell-k)}\alpha^{\ell-k}(r_1r_2)^\frac{\ell+k}{n}\right)\right)\\\label{eqn:case2:1}
& +n^2e^{-n(|z_1|^\frac{2}{n}+|z_2|^\frac{2}{n})}\sum\limits_{i,j=1}^{n}\left(\sum\limits_{\ell=k=0}^{n-1}\frac{n^{k+\ell}}{k!\ell!}(r_1r_2)^\frac{\ell+k}{n}\right)
\end{align}
The term \eqref{eqn:case2:1} doesnot contribute to the sum, because for fixed $\ell\neq k$ and $j$ the sum $\sum\limits_{i=1}^{n}\omega_n^{(\ell-k)(i-j)}=0$. Hence,
\begin{align}
\lim\limits_{n \rightarrow \infty}\frac{1}{n^4|z_1z_2|^{2-\frac{2}{n}}}\sum\limits_{i,j=1}^{n}|K(z_1^\frac{1}{n}\omega_i,z_2^\frac{1}{n}\omega_j)|^2 & = \lim\limits_{n \rightarrow \infty}\frac{n^2e^{-n(r_1^\frac{2}{n}+r_2^\frac{2}{n})}}{n^4(r_1r_2)^{2-\frac{2}{n}}}\sum\limits_{i,j=1}^{n}\left(\sum\limits_{\ell=k=0}^{n-1}\frac{n^{k+\ell}}{k!\ell!}(r_1r_2)^\frac{\ell+k}{n}\right)\\
& =\lim\limits_{n \rightarrow \infty}\frac{1}{\pi^2(r_1r_2)^{2-\frac{2}{n}}} \sum\limits_{\ell=0}^{n-1}\left(\frac{n^\ell e^{-n r_1^{\frac{2}{n}}}r_1^{\frac{2\ell}{n}}}{\ell!}\frac{n^\ell e^{-n r_2^{\frac{2}{n}}}r_2^{\frac{2\ell}{n}}}{\ell!}\right)\\
& \leq \lim\limits_{n \rightarrow \infty}\frac{1}{\pi^2(r_1r_2)^{2-\frac{2}{n}}} \sum\limits_{\ell=0}^{\infty}\left(\frac{n^\ell e^{-n r_1^{\frac{2}{n}}}r_1^{\frac{2\ell}{n}}}{\ell!}\frac{n^\ell e^{-n r_2^{\frac{2}{n}}}r_2^{\frac{2\ell}{n}}}{\ell!}\right)\\
& = \lim\limits_{n\rightarrow\infty}\frac{1}{\pi^2(r_1r_2)^{2-\frac{2}{n}}}\Pr\left(Y_1^{(n)}=Y_2^{(n)}\right)
\end{align}
Where $Y_1^{(n)}$ and $Y_2^{(n)}$ are independent Poisson random variables with means  $nr_1^\frac{2}{n}$ and $nr_2^\frac{2}{n}$ respectively. At the same time we can write each $Y_1^{(n)}$ and $Y_2^{(n)}$ as the sum of n-independent identical Poisson random variables whose means are $r_1^\frac{2}{n}$ and $r_2^\frac{2}{n}$ respectively. In other words $Y_1^{(n)}=P_1^{n}+P_2^{(n)}+\dots +P_n^{(n)}$, $Y_2^{(n)}=Q_1^{(n)}+Q_2^{(n)}+\dots+Q_n^{(n)}$ where $P_i^{(n)}$s and $Q_i^{(n)}$s are independent Poisson random variables with means $r_1^{\frac{2}{n}}$ and $r_2^\frac{2}{n}$ respectively. We will show that
$$
\lim\limits_{n\rightarrow\infty}\frac{1}{\pi^2(r_1r_2)^{2-\frac{2}{n}}}\Pr\left(Y_1^{(n)}-Y_2^{(n)}\right)=0 \label{eqn:case2:3}
$$
Once we prove \eqref{eqn:case2:3} we will have
$$\rho_2'(z_1,z_2)=\lim\limits_{n\rightarrow\infty}\rho_{2,n}'(z_1,z_2)=\lim\limits_{n\rightarrow\infty}\dfrac{n^2K(z_1^\frac{2}{n},z_1^\frac{2}{n})K(z_2^\frac{2}{n},z_2^\frac{2}{n})}{n^4|z_1z_2|^{2-\frac{2}{n}}}=\frac{1}{(2\pi)^2|z_1z_2|^2}=\rho_1'(z_1)\rho_1'(z_2)$$

Now it remains to prove \eqref{eqn:case2:3}. We shall state Lynaponav central limit theorem and show that the triangular array $P_i^{(n)}-Q_i^{(n)}$ satisfies the hypothesis of Lyapunov central limit theorem and use this to show \eqref{eqn:case2:3}. 
\begin{theorem}[Lyaponov CLT \cite{billingsley}]
Let $\{X_{i,n}\}$ be a triangular array of random variables with i.i.d random variables in each row and let $s_n^2=\sum\limits_{i=1}^{n}Var(X_{i,n})$, $S_n=\sum\limits_{i=1}^{n}X_{i,n}$. If $ \lim\limits_{n\rightarrow\infty}\dfrac{\sum\limits_{i=1}^{n}\text{$\mathbb{E}$}|X_{i,n}-\text{$\mathbb{E}$}(X_{i,n})|^{2+\delta}}{s_n^{2+\delta}}=0$ for some $\delta>0$ then as $n$ approaches to infinity the random variables $\dfrac{S_n-\text{$\mathbb{E}$}(S_n)}{s_n}$  converges in distribution to $N(0,1)$. $$\dfrac{S_n-\text{$\mathbb{E}$}(S_n)}{s_n}\xrightarrow{d} N(0,1)$$.  
\end{theorem}
For showing the hypothesis of Lyaponov CLT is satisfied choose $X_{i,n}=P_i^{(n)}-Q_i^{(n)}$. Then $$s_n^4=\left(\sum\limits_{i=1}^{n}Var(X_{i,n})\right)^2=\left(\sum\limits_{i=1}^{n}Var(P_i^{(n)}-Q_i^{(n)})\right)^2=\left(\sum\limits_{i=1}^{n}\left(Var(P_i^{(n)})+Var(Q_i^{(n)})\right)\right)^2=n^2(r_1^\frac{2}{n}+r_2^\frac{2}{n})^2$$ and  $$\text{$\mathbb{E}$}\left(P_i^{(n)}+Q_i^{(n)}-\text{$\mathbb{E}$}(P_i^{(n)}+Q_i^{(n)})\right)^4=\left(r_1^\frac{2}{n}+r_2^\frac{2}{n}\right)\left(3(r_1^\frac{2}{n}+r_2^\frac{2}{n})+4\right)$$.
Therefore
$$
\lim\limits_{n\rightarrow\infty}\dfrac{\sum\limits_{i=1}^{n}\text{$\mathbb{E}$}|X_{i,n}-\text{$\mathbb{E}$}(X_{i,n})|^{2+2}}{s_n^{2+2}} = \lim\limits_{n\rightarrow\infty}\dfrac{n\left(r_1^\frac{2}{n}+r_2^\frac{2}{n}\right)\left(3(r_1^\frac{2}{n}+r_2^\frac{2}{n})+4\right)}{n^2\left(r_1^\frac{2}{n}+r_2^\frac{2}{n}\right)^2}=0
$$
So $\dfrac{Y_1^{(n)}-Y_2^{(n)}-n(r_1^\frac{2}{n}-r_2^\frac{2}{n})}{\sqrt{n(r_1^\frac{2}{n}+r_2^\frac{2}{n})}}\xrightarrow{d}N(0,1)$. Observing that $\lim\limits_{n \rightarrow \infty}\sqrt{n}(r_1^\frac{2}{n}-r_2^\frac{2}{n})=0$ and $\lim\limits_{n\rightarrow \infty}(r_1^\frac{2}{n}+r_2^\frac{2}{n})=2$ we get $\dfrac{Y_1^{(n)}-Y_2^{(n)}}{\sqrt{n}}\xrightarrow{d}N(0,2)$. From the above facts we obtain

\begin{align}
 \lim\limits_{n\rightarrow\infty}\Pr(Y_1^{(n)}-Y_2^{(n)}=0)
  & \leq\lim\limits_{n\rightarrow\infty}\Pr(|Y_1^{(n)}-Y_2^{(n)}|<1)\\
 &=\lim\limits_{n\rightarrow\infty}\Pr\left(\frac{|Y_1^{(n)}-Y_2^{(n)}|}{\sqrt{n}}<\frac{1}{\sqrt{n}}\right)
 =0
\end{align}
Hence we have shown that \eqref{eqn:case2:3} is satisfied and verified the case k=2.
 



 


\subsubsection{Case:Arbitrary-$k$}
For proving the result for $k \geq 2$, we need to 
Like in the previous cases let us define $z_j=r_j\alpha_j$ for $j=1,2,\dots,k$ where $|\alpha_j|=1$.

\begin{align}
\rho_{k,n}'(z_1,z_2,\dots,z_k) & =\frac{\sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\rho_{k,n}(z_1^{\frac{1}{n}}\omega_n^{i_1},z_2^{\frac{1}{n}}\omega_n^{i_2},\dots,z_k^{\frac{1}{n}}\omega_n^{i_k})}{n^{2k}|z_1z_2\dots z_k|^{2-\frac{2}{n}}}\\
& = \frac{\sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\det\left(\left(K(z_\ell^{\frac{1}{n}}\omega_n^{i_\ell},z_m^{\frac{1}{n}}\omega_n^{i_m})\right)\right)_{1\leq\ell,m\leq k}}{n^{2k}|z_1z_2\dots z_k|^{2-\frac{2}{n}}}\\
& = \frac{\sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\sum\limits_{\sigma \in S_k} sgn(\sigma) \prod\limits_{s=1}^{k}K(z_s^{\frac{1}{n}}\omega_n^{i_s},z_{\sigma(s)}^{\frac{1}{n}}\omega_n^{i_{\sigma(s)}})}{n^{2k}|z_1z_2\dots z_k|^{2-\frac{2}{n}}}\\
& = \frac{\sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\sum\limits_{\sigma \in S_k} sgn(\sigma) \prod\limits_{s=1}^{k}\sum\limits_{j=0}^{k-1}\frac{n^j}{j!}(r_sr_{\sigma(s)}\alpha_s\overline{\alpha_{\sigma(s)}})^\frac{j}{n}\omega_n^{j(i_s-i_{\sigma(s)})}\times ne^{-(r_s^\frac{2}{n}+r_{\sigma(s)}^\frac{2}{n})/2}}{n^{2k}|z_1z_2\dots z_k|^{2-\frac{2}{n}}}\\
& =\sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\dfrac{n^ke^{-(r_1^\frac{2}{n}+\dots+r_k^\frac{2}{n})}}{n^{2k}\pi^k|z_1z_2\dots z_k|^{2-\frac{2}{n}}} 
\sum\limits_{\sigma \in S_k} sgn(\sigma)\prod\limits_{s=1}^{k}\left(\sum\limits_{j=0}^{k-1}(r_sr_{\sigma(s)})^\frac{j}{n}\omega_n^{j(i_s-i_{\sigma(s)})}(\alpha_s\overline{\alpha_{\sigma(s)}})^\frac{j}{n}\frac{n^j}{j!}\right)\label{eqn:perm}\\
\end{align}
Expanding the product in \ref{eqn:perm} we get
\begin{align}
\sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\dfrac{n^ke^{-(r_1^\frac{2}{n}+\dots+r_k^\frac{2}{n})}}{n^{2k}\pi^k|z_1z_2\dots z_k|^{2-\frac{2}{n}}}  \sum\limits_{\sigma \in S_k}sgn(\sigma)\sum\limits_{j_1,j_2,\dots,j_k=0}^{k-1}\dfrac{n^{(j_1+j_2+\dots+j_k)}}{j_1!j_2!\dots j_k!}\prod\limits_{\ell=1}^{k}(r_\ell r_{\sigma(\ell)}\alpha_\ell\overline{\alpha_{\sigma(\ell)}})^{\frac{j_\ell}{n}}\omega_n^{j_\ell(i_\ell-i_{\sigma(\ell)})}\label{eqn:perm1} 
\end{align}
Let $\sigma=C_1C_2\dots C_\ell$ where $C_1,C_2,\dots ,C_\ell$ are disjoint cycles of $\sigma$. Then \ref{eqn:perm1} will be reduced to\\
***************************************\\
need more explanation\\
***************************************\\
\begin{align}
\sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\dfrac{e^{-(r_1^\frac{2}{n}+\dots+r_k^\frac{2}{n})}}{n^{k}|z_1z_2\dots z_k|^{2-\frac{2}{n}}}\sum\limits_{\sigma \in S_n}sgn(\sigma)\sum\limits_{j_{k_1},j_{k_2},\dots,j_{k_\ell}=0}^{k-1}\prod\limits_{v=1}^{\ell}\prod\limits_{u\in C_i}(r_u r_{\sigma(u)})^{j_{k_v}}\frac{n^{j_{k_v}}}{j_{k_v}!}
\end{align}

%A typical term in the above term \ref{eqn:perm} is
%\begin{align}
%&\sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\dfrac{n^ke^{-(r_1^\frac{2}{n}+\dots+r_k^\frac{2}{n})}}{n^{2k}\pi^k|z_1z_2\dots z_k|^{2-\frac{2}{n}}} 
%  \prod\limits_{s=1}^{k}\left(\sum\limits_{j=0}^{k-1}(r_sr_{\sigma(s)})^\frac{j}{n}\omega_n^{j(i_s-i_{\sigma(s)})}(\alpha_s\overline{\alpha_{\sigma(s)}})^\frac{j}{n}\frac{n^j}{j!}\right)&\\
%& = \sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\dfrac{n^ke^{-(r_1^\frac{2}{n}+\dots+r_k^\frac{2}{n})}}{n^{2k}\pi^k|z_1z_2\dots z_k|^{2-\frac{2}{n}}}  \sum\limits_{j_1,j_2,\dots,j_k=0}^{k-1}\dfrac{n^{(j_1+j_2+\dots+j_k)}}{j_1!j_2!\dots j_k!}&\\ &  \times(r_1r_{\sigma(1)}\alpha_1\overline{\alpha_{\sigma(1)}})^{\frac{j_1}{n}}\dots(r_kr_{\sigma(k)}\alpha_k\overline{\alpha_{\sigma(k)}})^\frac{j_k}{n}\omega_n^{j_1(i_1-i_{\sigma(1)})+\dots+j_k(i_k-i_{\sigma(k)})}\\
%& = \sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\dfrac{n^ke^{-(r_1^\frac{2}{n}+\dots+r_k^\frac{2}{n})}}{n^{2k}\pi^k|z_1z_2\dots z_k|^{2-\frac{2}{n}}} \sum\limits_{\substack{j_1,j_2,\dots,j_{k_1}\\
%j_{k_1+1},j_{k_1+2},\dots,j_{k_2}\\
%\vdots\\ 
%j_{k_{r-1}+1},j_{k_{r-1}+2},\dots,j_{k_r}
%}=0}^{k-1}\dfrac{n^{(j_1+j_2+\dots+j_k)}}{j_1!j_2!\dots j_k!}\\
%& = \sum\limits_{i_1,i_2,\dots,i_k=1}^{n}\dfrac{n^ke^{-(r_1^\frac{2}{n}+\dots+r_k^\frac{2}{n})}}{n^{2k}\pi^k|z_1z_2\dots z_k|^{2-\frac{2}{n}}} \sum\limits_{\substack{j_1,j_2,\dots,j_{k_1}\\
%j_{k_1+1},j_{k_1+2},\dots,j_{k_2}\\
%\vdots\\ 
%j_{k_{r-1}+1},j_{k_{r-1}+2},\dots,j_{k_r}
%}=0}^{k-1}\dfrac{n^{(j_1+j_2+\dots+j_k)}}{j_1!j_2!\dots j_k!}&\\ 
%\end{align}

\section{Result}

